Detecting Adversarial Samples from Artifacts

Deep neural networks (DNNs) are powerful nonlinear architectures that are known to be robust to random perturbations of the input. However, these models are vulnerable to adversarial perturbations--small input changes crafted explicitly to fool the model. In this paper, we ask whether a DNN can distinguish adversarial samples from their normal and noisy counterparts. We investigate model confidence on adversarial samples by looking at Bayesian uncertainty estimates, available in dropout neural networks, and by performing density estimation in the subspace of deep features learned by the model. The result is a method for implicit adversarial detection that is oblivious to the attack algorithm. We evaluate this method on a variety of standard datasets including MNIST and CIFAR-10 and show that it generalizes well across different architectures and attacks. Our findings report that 85-93% ROC-AUC can be achieved on a number of standard classification tasks with a negative class that consists of both normal and noisy samples.

==> undecided_classification.tex <==
\section{Undecided Classification}
Following our findings in section 3, we formulate a new classification framework that uses model uncertainty to filter out low confidence samples for further analysis. Then, we evaluate this framework empirically on MNIST and CIFAR-10.
\subsection{Approach}
For a model with $C$ classes, we extend the model's predictions to include an \textit{undecided} class, leaving a total of $C+1$ possible predictions. Our goal is to find an uncertainty threshold during training above which any sample will be classified as undecided at test time. Given a trained model $M$ and a validation set $X_{valid}, Y_{valid}$ with $N$ samples, we apply the FGSM method to craft $N$ adversarial samples by perturbing the inputs in $X_{valid}$. Thereafter, we compute uncertainty estimates for each of the $N$ adversarial samples, and set our uncertainty threshold at percentile $P$, where $P$ is an algorithm parameter. This approach is described in Algorithm \ref{alg:threshold}. Note that algorithm parameter $P$ can be decided on analytically, after observing uncertainty distributions for each sample type. For the example shown in Figure \ref{fig:uncertainty_distribution}, we might choose $P=25\%$ as a good starting point.
\begin{algorithm}[h]
   \caption{Determine an uncertainty threshold}
   \label{alg:threshold}
\begin{algorithmic}
   \STATE {\bfseries Input:} model $M$, validation data $(X_{valid},Y_{valid})$, percentile $P$
   \STATE $X^* \gets \operatorname{Adversarial}(M,X_{valid},Y_{valid})$
   \STATE $U \gets \operatorname{Uncertainty}(M,X^*)$
   \STATE RETURN $\operatorname{Percentile}(U, P)$
\end{algorithmic}
\end{algorithm}

After determining our uncertainty threshold, we follow a simple classification rule using this value. At test time, samples that fall under the uncertainty threshold are classified with the model's prediction, and those that fall above the threshold are classified as undecided. This method is depicted in Algorithm \ref{alg:approach1}.

\begin{algorithm}[h]
   \caption{Threshold on uncertainty}
   \label{alg:approach1}
\begin{algorithmic}
   \STATE {\bfseries Input:}$(X_{train}, Y_{train})$, $(X_{valid}, Y_{valid})$, $X_{test}$
   \STATE $M \gets \operatorname{Train}(X_{train}, Y_{train})$
   \STATE cutoff $\gets \operatorname{Uncertainty\_threshold}(M, X_{valid}, Y_{valid})$
   \FOR{$x$ in $X_{test}$}
   \STATE $U = \operatorname{Uncertainty}(M, x)$
   \IF{$U >$ cutoff}
   \STATE prediction $\gets$ undecided
   \ELSE
   \STATE $P \gets \operatorname{Evaluate\_model(M, x)}$
   \STATE prediction $\gets \operatorname{arg\,max}_jP_j$
   \ENDIF
   \ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{Experiments}
\textit{TODO: put together concrete results for undecided classification w/ MNIST and CIFAR-10.}
